Hand-Object Interaction in the Age of Large Foundation Models:Reconstruction, Generation, and Embodied Transfer

Hand-object interaction (HOI) modeling remains challenging because it requires joint reasoning about hand articulation, object geometry, contact, semantics, and dynamics under severe visual uncertainty. Foundation models introduce transferable prior knowledge learned from large-scale cross-domain data, offering new ways to address these challenges beyond task-specific data and models. However, the rapidly growing literature remains fragmented, and existing studies typically describe these methods simply as ``using large models'' without systematically characterizing what knowledge is introduced, where it enters the HOI pipeline, or which HOI uncertainty it helps reduce. This survey presents the first systematic review of foundation-model priors for HOI. We organize the literature into six HOI tasks spanning reconstruction and generation. More importantly, we establish a taxonomy of eight foundation-model sub-priors grouped into geometric, semantic, and visual families. Geometric priors encompass shape retrieval, shape reconstruction, and spatial reconstruction; semantic priors include semantic grounding and language reasoning; and visual priors cover visual representation, image generation, and video generation. Based on this taxonomy, we systematically analyze how different priors are represented, injected, and adapted across HOI pipelines and tasks. Beyond how foundation models empower HOI, we further examine how HOI-derived knowledge is used in robot learning, including human-data pretraining, human-to-robot skill transfer, and HOI-to-robot data generation. Finally, we summarize datasets and evaluation protocols, and discuss limitations and future directions toward more generalizable HOI systems. To support long-term progress, we curate a live repository that continuously aggregates emerging methods and benchmarks.

==> figures/fig_example.tex <==
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=\linewidth]{Images/teaser.jpg}
  \end{center}
  \caption{\small Figure caption.}
  \label{fig:label}
\end{figure}

==> figures/fig_prior_task.tex <==
% \begin{figure*}[!t]
% \centering
% \includegraphics[width=\textwidth]{figures/priors-sections-tasks-h.pdf}
% \caption{Taxonomy roadmap of this survey. Three foundation-model prior families are decomposed into section-level sub-priors and linked to the HOI reconstruction or generation tasks reviewed under each subsection.}
% \label{fig:priors-sections-tasks}
% \end{figure*}

\begin{figure*}[t]
\centering

\begin{tikzpicture}[
    basebox/.style={
        rounded corners=3mm,
        line width=0.7pt,
        text width=6cm,
        minimum height=1.25cm,
        align=left,
        anchor=north west,
        inner xsep=1mm,
        inner ysep=1mm,
        font=\small
    }
]

% 第一行
\node[
    basebox,
    text width=8cm,
    draw=cyan!80,
    fill=cyan!0
] (box1) at (-4,0) {
    \textbf{C1}: Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA}
};

\node[
    basebox,
    text width=8cm,
    draw=blue!65!black,
    fill=blue!0
] (box2) at (5,0) {
    \textbf{C2}: Method B (\textit{ICCV} 2023)~\cite{methodB}
};

% 第二行
\node[
    basebox,
    text width=8cm,
    draw=red!65!black,
    fill=red!0
] (box3) at (-4,-1.8) {
    \textbf{C3}: Method C (\textit{NeurIPS} 2024)~\cite{methodC}
};

\node[
    basebox,
    text width=8cm,
    draw=orange!75!black,
    fill=orange!0
] (box4) at (5,-1.8) {
    \textbf{C4}: Method D (\textit{ICRA} 2025)~\cite{methodD}
};

% 第三行
\node[
    basebox,
    text width=8cm,
    draw=purple!65!black,
    fill=purple!0
] (box5) at (-4,-3.6) {
    \textbf{C5}: Method E (\textit{CoRL} 2023)~\cite{methodE}
};

\node[
    basebox,
    text width=8cm,
    draw=cyan!65!black,
    fill=cyan!0
] (box6) at (5,-3.6) {
    \textbf{C6}: Method F (\textit{IROS} 2024)~\cite{methodF}
};

% 第四行
\node[
    basebox,
    text width=8cm,
    draw=teal!70!black,
    fill=teal!0
] (box7) at (-4,-5.4) {
    \textbf{C7}: Method G (\textit{CVPR} 2025)~\cite{methodG}
};

\node[
    basebox,
    text width=8cm,
    draw=magenta!65!black,
    fill=magenta!0
] (box8) at (5,-5.4) {
    \textbf{C8}: Method H (\textit{RSS} 2024)~\cite{methodH}
};

% 第五行
\node[
    basebox,
    text width=8cm,
    draw=yellow!60!black,
    fill=yellow!0
] (box9) at (-4,-7.2) {
    \textbf{C9}: Method I (\textit{RA-L} 2025)~\cite{methodI}
};

\node[
    basebox,
    text width=8cm,
    draw=gray!70!black,
    fill=gray!0
] (box10) at (5,-7.2) {
    \textbf{C10}: Method J (\textit{arXiv} 2025)~\cite{methodJ}
};

\end{tikzpicture}

\caption{Representative methods.}
\label{fig:method-boxes}
\end{figure*}

==> figures/fig_prior_task_all_method.tex <==
\begin{figure*}[t]
\centering

\begin{subfigure}[t]{\textwidth}
    \centering
    \includegraphics[
        width=\textwidth
    ]{figures/priors-sections-tasks-h.pdf}
    % \caption{}
    \label{fig:taxonomy}
\end{subfigure}

\begin{subfigure}[t]{\textwidth}
    \centering
    \begin{tikzpicture}[
    basebox/.style={
        rounded corners=3mm,
        line width=0.7pt,
        text width=6cm,
        minimum height=1.25cm,
        align=left,
        anchor=north west,
        inner xsep=1mm,
        inner ysep=1mm,
        font=\small
    }
]

    % 第一行
    \node[
        basebox,
        text width=8cm,
        draw=cyan!80,
        fill=cyan!0
    ] (box1) at (-4,0) {
        \textbf{C1}: Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA},Method A (\textit{CVPR} 2024)~\cite{methodA}
    };
    
    \node[
        basebox,
        text width=8cm,
        draw=blue!65!black,
        fill=blue!0
    ] (box2) at (5,0) {
        \textbf{C2}: Method B (\textit{ICCV} 2023)~\cite{methodB}
    };
    
    % 第二行
    \node[
        basebox,
        text width=8cm,
        draw=red!65!black,
        fill=red!0
    ] (box3) at (-4,-1.8) {
        \textbf{C3}: Method C (\textit{NeurIPS} 2024)~\cite{methodC}
    };
    
    \node[
        basebox,
        text width=8cm,
        draw=orange!75!black,
        fill=orange!0
    ] (box4) at (5,-1.8) {
        \textbf{C4}: Method D (\textit{ICRA} 2025)~\cite{methodD}
    };
    
    % 第三行
    \node[
        basebox,
        text width=8cm,
        draw=purple!65!black,
        fill=purple!0
    ] (box5) at (-4,-3.6) {
        \textbf{C5}: Method E (\textit{CoRL} 2023)~\cite{methodE}
    };
    
    \node[
        basebox,
        text width=8cm,
        draw=cyan!65!black,
        fill=cyan!0
    ] (box6) at (5,-3.6) {
        \textbf{C6}: Method F (\textit{IROS} 2024)~\cite{methodF}
    };
    
    % 第四行
    \node[
        basebox,
        text width=8cm,
        draw=teal!70!black,
        fill=teal!0
    ] (box7) at (-4,-5.4) {
        \textbf{C7}: Method G (\textit{CVPR} 2025)~\cite{methodG}
    };
    
    \node[
        basebox,
        text width=8cm,
        draw=magenta!65!black,
        fill=magenta!0
    ] (box8) at (5,-5.4) {
        \textbf{C8}: Method H (\textit{RSS} 2024)~\cite{methodH}
    };
    
    % 第五行
    \node[
        basebox,
        text width=8cm,
        draw=yellow!60!black,
        fill=yellow!0
    ] (box9) at (-4,-7.2) {
        \textbf{C9}: Method I (\textit{RA-L} 2025)~\cite{methodI}
    };
    
    \node[
        basebox,
        text width=8cm,
        draw=gray!70!black,
        fill=gray!0
    ] (box10) at (5,-7.2) {
        \textbf{C10}: Method J (\textit{arXiv} 2025)~\cite{methodJ}
    };
    
    \end{tikzpicture}
    
        % \caption{Representative methods categorized by HOI tasks.}
        \label{fig:methods}
    \end{subfigure}

\caption{
Taxonomy roadmap of this survey. Three foundation-model prior families are decomposed into section-level sub-priors and linked to the HOI reconstruction or generation tasks reviewed under each subsection.
}
\label{fig:overview}
\end{figure*}


==> sections/0_abs.tex <==
\begin{abstract}
Here is the abstract.
\end{abstract}


==> sections/1_intro.tex <==
\section{Introduction}
Here is an introduction with citations \cite{bib:mobrecon,bib:bert,bib:smpl}.


==> sections/2_relate.tex <==
\section{Related Work}
Here is the related works.


==> sections/3_method.tex <==
\section{Method}
Here is the Method.


==> sections/4_exp.tex <==
\section{Experiments}
As shown in \autoref{fig:label} and \autoref{tab:table}, here is the experiment.

\input{Figures/fig_example}

\input{Tables/tab_example}


==> sections/5_con.tex <==
\section{Conclusion}
Here is the conclusion.

\section*{Acknowledgements}
Acknowledgements can include anyone who contributed through discussions,
feedback on drafts, implementation, or other support.


==> sections/X_app.tex <==
\section{Appendix}
Here is the appendix.

==> tables/tab_example.tex <==
\begin{table}[!t]
  \caption{Sample table title}
  \centering
  \begin{tabular}{lll}
    \toprule
    Name & Description & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal & $\sim$100 \\
    Axon & Output terminal & $\sim$10 \\
    Soma & Cell body & up to $10^6$ \\
    \bottomrule
  \end{tabular}
  \label{tab:table}
\end{table}

==> tables/table-representative-methods-ieee-original.tex <==
\begin{table*}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}
\caption{Representative foundation-model-prior methods for HOI. P and A denote primary and auxiliary prior sources, respectively. A source is primary when it supplies the task-defining representation or intervention that determines the method's placement in this survey; sources used for upstream perception, conditioning, alignment, or refinement are auxiliary.}
\label{tab:representative-fm-methods}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{0.13\textwidth}>{\raggedright\arraybackslash}p{0.09\textwidth}>{\raggedright\arraybackslash}p{0.16\textwidth}YY>{\raggedright\arraybackslash}p{0.18\textwidth}@{}}
\toprule
Method & Status & Task & Foundation-model prior source & Injected representation & Injection operator \\
\midrule
\multicolumn{6}{@{}l}{\textit{Primary family: Geometric priors} (\autoref{sec:3d-geometry-priors})} \\
\midrule
EasyHOI~\cite{liu2025easyhoi} & CVPR 2025 & R2: Hand-Held Object Reconstruction & \textbf{P}: InstantMesh~\cite{xu2024instantmesh}; \textbf{A}: LISA~\cite{lai2024lisa}, SAM~\cite{kirillov2023segment}, Affordance Diffusion~\cite{ye2023affordance} & region masks; inpainted object image; object mesh & grounding; shape initialization \\
GraG~\cite{aytekin2026grasp} & arXiv 2026 & R3: Dynamic HOI Reconstruction & \textbf{P}: SAM~3D~\cite{chen2026sam}, MV-SAM3D~\cite{li2026mv}; \textbf{A}: SAM~3~\cite{carion2025sam} & region masks; canonical object mesh & grounding; shape initialization \\
MCC-HO~\cite{wu2026reconstructing} & 3DV 2026 & R2: Hand-Held Object Reconstruction & \textbf{P}: Luma AI Genie~\cite{lumalabs}; \textbf{A}: GPT-4V~\cite{gpt4vsystemcard}, DINOv2~\cite{oquab2023dinov2} & object description; generated object mesh; image features & shape initialization; alignment \\
GHOST~\cite{aboukhadra2026ghost} & CVPR 2026 & R2: Hand-Held Object Reconstruction & \textbf{P}: OpenShape~\cite{liu2023openshape}; \textbf{A}: SAM~2~\cite{ravi2025sam}, InternVL~\cite{chen2024internvl} & region mask; object identity; retrieved 3D asset & grounding; retrieval/alignment \\
HOSt3R~\cite{swamy2025host3r} & ICCV Workshop 2025 & R1: Hand-Object Pose Estimation & \textbf{P}: DUSt3R~\cite{wang2024dust3r} & point maps; 3D transforms & geometry fusion \\
EgoGrasp~\cite{fu2026egograsp} & arXiv 2026 & R3: Dynamic HOI Reconstruction & \textbf{P}: Depth Anything~3~\cite{lin2025depth}, SAM~3D~\cite{chen2026sam}; \textbf{A}: SAM~2~\cite{ravi2025sam} & metric depth; region mask; object mesh & geometry fusion \\
ArtHOI~\cite{wang2026arthoi} & CVPR 2026 & R3: Dynamic HOI Reconstruction & \textbf{P}: Video-Depth-Anything~\cite{chen2025video}, UniDepth~V2~\cite{piccinelli2025unidepthv2}, Hunyuan3D~\cite{lai2025hunyuan3d}; \textbf{A}: SAM~2~\cite{ravi2025sam}, Qwen-VL-Max~\cite{bai2023qwen} & metric depth; camera parameters; region masks; object mesh; contact cues & geometry fusion; constraint/scoring; visual editing \\
\midrule
\multicolumn{6}{@{}l}{\textit{Primary family: Semantic priors} (\autoref{sec:semantic-priors})} \\
\midrule
CHOIR~\cite{xu2026choir} & arXiv 2026 & R3: Dynamic HOI Reconstruction & \textbf{P}: SAM~2~\cite{ravi2025sam}, Amodal Video Segmenter~\cite{chen2025using}; \textbf{A}: SAM~3D~\cite{chen2026sam}, MoGe-2~\cite{wang2026moge} & amodal masks; canonical object mesh; metric depth; object scale & grounding; shape initialization; geometry fusion \\
Text2Grasp~\cite{chang2025text2grasp} & ISNN 2025 & G1: Hand-Object Grasp Synthesis & \textbf{P}: GPT-3~\cite{brown2020language}, CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21} & task-part plan; grasp description & constraint/scoring \\
SemGrasp~\cite{li2024semgrasp} & ECCV 2024 & G1: Hand-Object Grasp Synthesis & \textbf{P}: Vicuna~\cite{vicuna2023}, GPT-4~\cite{achiam2023gpt}, GPT-4V~\cite{gpt4vsystemcard}, CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21} & grasp tokens; grasp description & constraint/scoring \\
NL2Contact~\cite{zhang2024nl2contact} & ECCV 2024 & G1: Hand-Object Grasp Synthesis & \textbf{P}: ChatGPT~\cite{chatgpt}, BERT~\cite{devlin2019bert} & contact description; text embedding & constraint/scoring \\
Afford\-Grasp~\cite{wu2026affordgrasp} & CVPR 2026 & G1: Hand-Object Grasp Synthesis & \textbf{P}: RoBERTa~\cite{liu2019roberta}, Qwen2~\cite{yang2024qwen2technicalreport} & multimodal condition embedding & constraint/scoring \\
Text2HOI~\cite{cha2024text2hoi} & CVPR 2024 & G2: HOI Motion Generation & \textbf{P}: CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21} & multimodal condition embedding & constraint/scoring \\
TOUCH~\cite{han2025touch} & arXiv 2025 & G2: HOI Motion Generation & \textbf{P}: Qwen-7B~\cite{bai2023qwentech} & coarse-to-fine condition tokens & constraint/scoring \\
\midrule
\multicolumn{6}{@{}l}{\textit{Primary family: Visual priors} (\autoref{sec:generative-priors})} \\
\midrule
HOI\-Diffusion~\cite{zhang2024hoidiffusion} & CVPR 2024 & G3: HOI Image/Video Generation & \textbf{P}: Stable Diffusion~\cite{rombach2022high}; \textbf{A}: CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21}, ChatGPT~\cite{chatgpt}, LLaVA~\cite{liu2023visual} & multiscale structural features; text embedding & weight initialization/fine-tuning; adapter conditioning \\
Prompt-Propose-Verify~\cite{juneja2023prompt} & arXiv 2023 & G3: HOI Image/Video Generation & \textbf{P}: SDXL~\cite{podell2024sdxl}; \textbf{A}: CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21}, GPT-4~\cite{achiam2023gpt} & enriched text prompt; visual latent & weight initialization/fine-tuning \\
SViMo~\cite{dang2025svimo} & NeurIPS 2025 & G3: HOI Image/Video Generation & \textbf{P}: CogVideoX-5B~\cite{yang2025cogvideox}; \textbf{A}: Google T5~\cite{raffel2020exploring} & tri-modal tokens; interaction embedding & weight initialization/fine-tuning; adapter conditioning \\
iDiT-HOI~\cite{shen2025idit} & arXiv 2025 & G3: HOI Image/Video Generation & \textbf{P}: Wan-14B I2V~\cite{wan2025wan}; \textbf{A}: FLUX.1-dev~\cite{DBLP:journals/corr/abs-2506-15742} & inpainting condition tokens & weight initialization/fine-tuning \\
\bottomrule
\end{tabularx}
\end{table*}

